Proving Correctness and Completeness of Normal Programs - a Declarative Approach

We advocate a declarative approach to proving properties of logic programs. Total correctness can be separated into correctness, completeness and clean termination; the latter includes non-floundering. Only clean termination depends on the operational semantics, in particular on the selection rule. We show how to deal with correctness and completeness in a declarative way, treating programs only from the logical point of view. Specifications used in this approach are interpretations (or theories). We point out that specifications for correctness may differ from those for completeness, as usually there are answers which are neither considered erroneous nor required to be computed. We present proof methods for correctness and completeness for definite programs and generalize them to normal programs. For normal programs we use the 3-valued completion semantics; this is a standard semantics corresponding to negation as finite failure. The proof methods employ solely the classical 2-valued logic. We use a 2-valued characterization of the 3-valued completion semantics which may be of separate interest. The presented methods are compared with an approach based on operational semantics. We also employ the ideas of this work to generalize a known method of proving termination of normal programs.

==> 56.tex <==

\section{Related work}

In this section we present a brief overview of related work.

Due to our approach to specifications,
we do not need any explicit
notion of precondition, type information, or domain of a procedure.
Such notions are used in most other approaches
\cite{BC89,Apt-Prolog,PR99,Deville} in order
to deal with ``ill-typed'' atoms, for which the behaviour of the
program is of no interest. 
For similar purposes Naish  \shortcite{naish:sem3} introduces
a 3-valued approach to definite programs.

An approach related to ours is 
the annotation method of Deransart
(\citeNP[Section~4]{Der93}; \citeNP[Section~4]{BM97})
 for proving definite program correctness.
It can be seen as refinement of the natural method of Section
\ref{sec.def.sound},
where one proves more (but smaller) implications than those to be proved in
the natural method.


A  method for proving completeness of definite programs,
 similar to ours, was presented in \cite{DM93}.
Both approaches are compared in Section \ref{sec.def.compl}.


Comparison with the operational method \cite{BC89,Apt-Prolog,PR99}
for correctness of definite programs is given in Section
\ref{sec.operational}.
The operational method can be generalized to correctness of normal
programs
\cite{Apt95,PR99}; we present a comparison in Section
\ref{subsec.norm.comparison}.
We show that the correctness proving approaches presented in this paper are
stronger than the corresponding operational ones 
(as far as properties of program answers are concerned);
moreover our approach for normal programs is strictly stronger.
The method of \cite{PR99} includes proving completeness of normal
programs.  In Section \ref{subsec.norm.compl}
we show that it is strictly weaker than the method of Theorem
\ref{ThNormComplete}.
Also, the methods presented in this paper are, in our opinion, simpler
than the operational ones.
In particular, in the approach of \cite{PR99} one
has to prove correctness, completeness and termination together.
Due to this one  cannot use approximate specifications.




The comparisons formally show that it is not necessary to refer to
operational semantics in reasoning about declarative properties of programs.
Naish \citeyear{Naish96} presents a similar opinion;
he advocates 
a declarative view for a class of program properties which are often
treated as operational.






A related early work is \cite{Deville}.  It presents a method to develop
Prolog programs.  Their correctness and completeness follows from construction.
However the construction process consists of many stages and is rather
complicated.

Our approach to normal programs considers their 3-valued semantics,
in contrast to \cite{Deville,Apt95,PR99}
where 2-valued semantics is used.
The 3-valued completion semantics more precisely corresponds to
the operational semantics mainly used in practice
(negation as finite failure and SLDNF-resolution).
Introducing 3-valued semantics does not result in any difficulties:
our proof methods use only the standard 2-valued logic.

An important approach to proving properties of normal programs was
proposed by St\"{a}rk \shortcite{Staerk97}.  It deals with normal programs,
executed under Prolog selection rule.
Success, failure and termination are described by an inductive theory,
called the inductive extension of a program.
The theory can be seen as a
refinement of the notion of
program completion.    The program's properties of interest are
expressed as formulae and one has to prove that they are
consequences  of the theory.  
This is opposite to our approach where properties are
expressed as specifications and appear to the left of $\models$,
while a program (or a theory similar to program completion) appears to the
right of $\models$. 


Some properties, 
like ``for any $k$ there exists $l$ such that $P\models p(k,l)$'',
are expressible in the approach of \cite{Staerk97} but cannot be
expressed as interpretations in our approach.
To deal with such properties we need to use specifications which are theories,
not interpretations; we expect that our approach is also applicable to such
specifications.


The approach  of \cite{Staerk97}
includes clean termination and is equipped
with a tool to mechanically verify the proofs.  It is however bound to
Prolog selection rule.
The involved induction scheme is rather complicated; the scheme seems
difficult to use without computer support.
The purpose of our work is different: we are interested in the
declarative semantics and in basic methods, which can be widely
understood by programmers and used
-- possibly in an informal form -- in practical reasoning about actual
programs.






Ferrand and Deransart  \shortcite{Deransart.normal} presented a method of
proving correctness of normal programs.
(Their terminology is different; what they call ``partial completeness''
is, in our terminology, correctness for negative atomic queries.)
In contrast to our work they deal with the well-founded semantics
\cite{wfsem}.  Their specifications are thus Herbrand
interpretations.  
The validation conditions of their method consist of
conditions equivalent to 
those of Theorem
\ref{ThNormCorrect}, and of additional requirement
involving existence of a certain well-founded ordering of atoms.

Malfon \citeyear{Malfon} presented methods of proving
program completeness for three kinds of semantics, given by
the well-founded model, the least fixpoint of $\Phi_P$, and by
$\Phi_P\mathop\uparrow\omega$.
(Notice that the latter is not the Kunen semantics considered in this paper.)
Similarly to the previous case, the proposed sufficient conditions for
completeness are (equivalent to) the
conjunction of our conditions for correctness and
a condition involving a well-founded ordering.
The latter depends on the considered semantics.

\medskip 


\section{Conclusions}

This paper advocates declarative reasoning about 
logic programs.
We show how to prove correctness and completeness 
of definite and normal logic programs in a declarative way,
independently from any operational semantics.
This makes it possible to separate reasoning about
``logic'' from reasoning about ``control''.
The method for proving correctness of definite programs is not
new, however its usefulness has not been appreciated.
The methods for completeness and for correctness of normal programs are
a contribution of this work.

We refer to two specifications; one for
correctness and one for completeness.
This makes it possible to specify the program semantics
approximately, thus simplifying
the specifications and the proofs.
In this paper
specifications are interpretations, but the approach seems
applicable to specifications being theories.


The semantics of normal programs is 3-valued.
We do not however explicitly refer to 3-valued logic.  
Instead, a pair of 2-valued specifications plays a role of a
4-valued specification for correctness and a 3-valued specification for
completeness.
Also, 
we use a 2-valued characterization of the 3-valued
completion semantics, which may be of separate interest.

Approximate specifications are convenient not only when one deals with
program correctness and completeness.
We show how approximate specifications can be used to generalize
and simplify the
proof method of  \cite{AP93} for termination of normal programs.

Some authors suggest referring to operational semantics, in particular
to the form of call patterns under LD- (LDNF-) resolution, when
reasoning about correctness.  
We claim that our approach is
simpler.   We show formally that whatever can be
proved using the operational approach, can be proved in the approach
advocated here (as far as properties of program answers are
concerned).  For normal programs our approach is strictly stronger, for
definite programs the two approaches are equivalent.


The operational methods additionally prove some properties of the
operational semantics, which are outside of the scope of our approach.
Obviously, when such properties are of interest,
operational methods are indispensable.  Their importance should not be
neglected.  But as long as we are
interested in properties of computed answers (correctness and completeness),
and not in some details of computations
(like call patterns),
the declarative approach is sufficient.
Termination is an important operational property, which in contrast to
correctness and completeness depends on the selection rule.
But even for termination most approaches, like the method of  \cite{AP93},
do not 
explicitly refer to call patterns (except for the initial query).


If it were necessary to resort to  operational semantics in order
to prove basic program properties then logic programming would not
deserve to be called a declarative programming paradigm.
This work shows that this is not the case.


We believe that the presented proof methods are simple and natural.
We claim that they are
 a formalization of a style of thinking in which a
competent logic programmer reasons (or should reason) about her
programs. 
We believe that these methods, possibly treated informally, are
a valuable tool for actual everyday reasoning about real programs.
We believe that they should be used in teaching
logic programming.  

\medskip\noindent
{\small
{\bf Acknowledgement} \
The first author
% has been
was partly supported by the European Commission
% and by the Swiss Federal Office for Education and Science
within the 6th~Framework
% Programme project REWERSE number~506779 ({\tt http://rewerse.net}).
Programme project REWERSE ({\tt http://rewerse.net}).
\sloppy\par
}

